Identification of the cosmogenic $^{11}$C background in large volumes of liquid scintillators with Borexino

Cosmogenic radio-nuclei are an important source of background for low-energy neutrino experiments. In Borexino, cosmogenic $^{11}$C decays outnumber solar $pep$ and CNO neutrino events by about ten to one. Highly efficient identification of this background is mandatory for these neutrino analyses. We present here the details of the most consolidated strategy, used throughout Borexino solar neutrino measurements. It hinges upon finding the space-time correlations between $^{11}$C decays, the preceding parent muons and the accompanying neutrons. This article describes the working principles and evaluates the performance of this Three-Fold Coincidence (TFC) technique in its two current implementations: a hard-cut and a likelihood-based approach. Both show stable performances throughout Borexino Phases II (2012-2016) and III (2016-2020) data sets, with a $^{11}$C tagging efficiency of $\sim$90 % and $\sim$63-66 % of the exposure surviving the tagging. We present also a novel technique that targets specifically $^{11}$C produced in high-multiplicity during major spallation events. Such $^{11}$C appear as a burst of events, whose space-time correlation can be exploited. Burst identification can be combined with the TFC to obtain about the same tagging efficiency of $\sim$90 % but with a higher fraction of the exposure surviving, in the range of $\sim$66-68 %.

==> abbrev.tex <==
%%% Commands and settings

% Pages
%\newcommand{\emptypage}{\clearpage{\pagestyle{empty}\cleardoublepage}} % do we need empty pages to always start left pages? I don't think so: it is not a book

% Title
%\DeclareDocumentCommand{\Title}{o m}{\IfNoValueTF{#1}{\title{\bf #2}}{\title[#1]{\bf #2}}} % comer journal format have options: activate this to readapt everything!

% Authors: To be reviewd...
%\renewcommand\Authfont{\sf}
%\renewcommand\Affilfont{\sf\small}
%\renewcommand\Authsep{, }
%\renewcommand\Authand{, }
%\renewcommand\Authands{, }
%\DeclareDocumentCommand{\collaboration}{o m}{ % THIS MUST BE THE LAST "author"! Optional argument is a weblink
%	\renewcommand\Authand{\\for the }
%	\renewcommand\Authands{\\for the }
%	\IfNoValueTF{#1}{\author[ ]{#2}}{\author[ ]{\href{#1}{#2}}}
%}

% Linking acrodefs: PROBABLY TO NOT BE USED!
\newcommand{\acH}[1]{\hyperlink{#1}{\ac{#1}}}
\newcommand{\acL}[1]{\hypertarget{#1}{\acs{#1}}}
\newcommand{\acEmp}[1]{\emph{\acl{#1}} (\acs{#1})\acused{#1}}
\newcommand{\acEnq}[1]{``\acl{#1}'' (\acs{#1})\acused{#1}}
\newcommand{\acpEmp}[1]{\emph{\aclp{#1}} (\acsp{#1})\acused{#1}}
\newcommand{\acpEnq}[1]{``\aclp{#1}'' (\acsp{#1})\acused{#1}}

% Widebar: a nicer one
\makeatletter
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{%
  \begingroup
  \def\mathaccent##1##2{%
    \rel@kern{1.2}% empty space in the box before the letter
    \overline{\rel@kern{-1.1}\macc@nucleus\rel@kern{-0.1}}% extension early the start of the box (-: shortening), after the box (-: shortening)
    \rel@kern{0.1}% empty space in the box after the letter
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \macc@nested@a\relax111{#1}%
  \endgroup
}
\makeatother
% Wide accents with powers
\newcommand{\wideTo}[3][\widehat]{#1{#2}\,^{#3}}
\newcommand{\wHat}[1]{\widehat{#1}\,} % Wide hat

%abbreviations with a period:  e.g., i.e., p.e.
\newcommand{\ie}{i.e.\ }
\newcommand{\Ie}{I.e.\ }
\newcommand{\pe}{p.e.\xspace}
\newcommand{\upe}{[p.e.]\xspace}
\newcommand\Neu{{\it neutrino}\xspace}
\newcommand\burst{{\it burst}\xspace}
\newcommand\bfburst{\textbf{\textit{burst}}\xspace}

% Physics & math
\newcommand\A[2]{$^{#2}$#1\xspace} % atomic abbreviation
\newcommand\bfA[2]{$^\mathbf{#2}$\textbf{#1}\xspace} % atomic abbreviation, bold font
\def\Cel{\A{C}{11}} % example with C11
\def\bfCel{\bfA{C}{11}} % example with C11, bold font



==> preamble.tex <==


\smartqed  % flush right qed marks, e.g. at end of proof
%
\RequirePackage{graphicx}

% Geometry
\usepackage[a4paper]{geometry}

% Languages
\usepackage[german,italian,french,main=english]{babel}

% Document format
%\usepackage{appendix}

% Text
%\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{textcomp,upgreek}

% Citation
\usepackage{cite,mcite}

% Math & Physics
\usepackage{amsmath,amstext,amssymb,mathtools,slashed,cancel,turnstile,wasysym} %useful tool in trunstile: \ndtstile{<bottom>}{<top>}

% Tables
\usepackage{longtable,multirow,tabularx,colortbl}

% Graphics
\usepackage{graphicx,subfigure,picture,epstopdf}
\usepackage[format=hang,font={small,sf},labelfont={sf,bf}]{caption}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}
\graphicspath{{./}{images/}}

% Useful definition for the doc creation
\usepackage{xspace,xcolor}

% Coding
\usepackage{forarray,xparse,xkeyval,environ,ifthen}

%to fix the bug in svjour3
\newcounter{chapter}

% Linking
%\usepackage{url}
\usepackage[pdftex,colorlinks=true,linkcolor=blue,citecolor=red,urlcolor=purple]{hyperref}
\usepackage[noabbrev,capitalise]{cleveref}

% Authors
%\usepackage{authblk} % see abbrev.tex for the rules

% Drafting
\usepackage{todonotes} % for figures placeholders, can be removed at the end
\usepackage{lineno}

\input{abbrev.tex}




